SPECI-2: An open-source framework for predictive simulation of cloud-scale data-centres

We introduce Version 2 of SPECI, a system for predictive simulation modeling of large-scale data-centres, i.e. warehouse-sized facilities containing hundreds of thousands of servers, as used to provide cloud services.

==> abstract.tex <==
\fontsize{9}{11}\selectfont We introduce Version 2 of SPECI, a system for predictive simulation modeling of large-scale data-centres, i.e. warehouse-sized facilities containing hundreds of thousands of servers, as used to provide cloud services.


==> authors-blind.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Anonymous Authors\\
  \fontsize{9}{11}\selectfont
  \textit{Anonymous University}\\
  \fontsize{9}{11}\selectfont
  \textit{\{some\} @email}\\[12pt]
  %
  %
  % repeat previous group of commands here for further authors
}


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Ilango Leonardo Sriram, Dave Cliff\\
  \fontsize{9}{11}\selectfont
  \textit{Department of Computer Science, University of Bristol, United Kingdom}\\
  \fontsize{9}{11}\selectfont
  \textit{\{ilango, dc\} @cs.bris.ac.uk}\\[12pt]
  %
  %
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont Data Centre, Cloud Computing, Middleware, Normal Failure, Discrete Event Simulation.


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{SPECI-2}\\
% The Subtitle should have initial letters capitalized
\fontsize{13}{15}\selectfont \textit{An open-source framework for predictive simulation of cloud-scale data-centres}
}

